Metamorphic Security Testing for Web Systems

Security testing verifies that the data and the resources of software systems are protected from attackers. Unfortunately, it suffers from the oracle problem, which refers to the challenge, given an input for a system, of distinguishing correct from incorrect behavior. In many situations where potential vulnerabilities are tested, a test oracle may not exist, or it might be impractical due to the many inputs for which specific oracles have to be defined. In this paper, we propose a metamorphic testing approach that alleviates the oracle problem in security testing. It enables engineers to specify metamorphic relations (MRs) that capture security properties of the system. Such MRs are then used to automate testing and detect vulnerabilities. We provide a catalog of 22 system-agnostic MRs to automate security testing in Web systems. Our approach targets 39% of the OWASP security testing activities not automated by state-of-the-art techniques. It automatically detected 10 out of 12 vulnerabilities affecting two widely used systems, one commercial and the other open source (Jenkins).

==> catalog.tex <==
\section{A Catalog of Metamorphic Relations for Security Testing}

We have defined a catalog of Metamorphic Relations that enables automated security metamorphic testing.
We derived the catalog by considering the type of security test cases described in the OWASP security testing guidelines for Web applications. 
For each type of security test case we have identified one or more metamorphic relations that enables to determine the presence of the vulnerability targeted by the corresponding test case. 
If a metamorphic relation does not hold then the system is vulnerable.
Metamorphic relations capture high-level properties that generally hold on Web systems

 the presence of the vulnerability when it does not hold.
To build the metamorphic relation we have introduced a set of relational operators (functions) that capture common characteristics of Web and Android systems.







==> dataCollection.tex <==
\section{Data Collection}
\label{sec:dataCollection}

Metamorphic relations enable engineers to express abstract properties of the data, e.g. to specify that a URL that belongs to an input sequence observed 


n input sequence In this paper we propose a metamorphic testing approach for cybersecurity. 
The approach builds on a DSL for specifying metamorphic relations for software security, 
a set of predefined metamorphic relations targeting well known security vulnerabilities for Web systems,
a framework that automatically collects data required to perform metamorphic testing of the system under test,
and a metamorphic testing framework that automatically performs security testing based on the metamorphic relations and the collected data. 
To facilitate the specification of metamorphic relations we developed an editor for metamorphic relations 
based on xtext, a framework for the development of programming languages, 
which has been implemented as a plugin for the Eclipse IDE~\cite{web:eclipse}.


Figure~\ref{fig:approach} provides an overview of the approach. In Step 1 engineers select from the set of provided metamorphic relations, the one that should hold on the system under test from the provided set. Additionally (Step 1.a ) engineers can also specify new metamorphic relations in scripts written using the provided DSL.
In Step 2 engineers execute the data collection framework. The data collection framework consists of a set of Web crawlers that collect information about the system under test (e.g., the URLs that can be visited by an anonymous user) and store them in a data pool that is inspected during testing.
In Step 3 engineers execute the metamorphic testing framework. The framework automatically loads the data required by the metamorphic relations, generate new data as described by the relation and sends inputs and collect outputs from the system under test. To this end the framework compose the features provided by different Web testing libraries such as the Selenium Web testing framework~\cite{web:selenium} and the unirest http request and proxy library~\cite{web:unirest}.

Despite out approach relies on a DSL and a framework that include generic features that are expected to enable the testing of most Web systems, it integrates some optional activities that enable engineers to extend the provided features to tailor the testing process to the needs of the system under test. Optional activities are Step 1.b, 2.a and 3.a in Figure~\ref{}. In Step 1.b engineers extend the expressiveness of the provided DSL by implementing new Java APIs to be used in the MR scripts. In Step 2.a engineers implement and execute new data collection methods that enable them retrieving data that is not collected by the provided framework.
In Step 3.a engineers extend the framework to tailor it to the specific needs of the system (e.g., to deal with non standard input protocols, or to load the data collected by the new data collection methods implemented in Step 2.a).

The following sections provide the details of the building blocks of our approach: the DSL, the provided metamorphic relations, the data collection framework and the automated metamorphic testing framework.

\begin{figure}[htbp]
\includegraphics[width=8cm]{images/approach.pdf}
\caption{Metamorphic testing for cybersecurity.}
\label{fig:approach}
\end{figure}


\input{dsl.tex}





==> tables/OWASPten.tex <==
\begin{table}[tb]
\footnotesize
\caption{Vulnerability types addressed by SMRL \MRs}
\begin{center}
\begin{tabular}{|p{7cm}|p{1cm}|}
\hline
\textbf{Vulnerability type}			&\textbf{\#MRs}\\
\hline
Injection				&0\\
Broken Authentication	&6\\
Sensitive Data Exposure	&5\\
XML External Entities	&0\\
Broken Access Control	&7\\
Security Misconfiguration	&3\\
Cross-site scripting		&0\\
Insecure Deserialization	&0\\
Using Vulnerable Components	&1\\
Insufficient Logging or Monitoring	&0\\
\hline
\end{tabular}
\end{center}
\label{default}
\end{table}%


==> tables/comboExamplePictureGrammar.tex <==

\begin{figure*}[h!]
\begin{minipage}[b]{\textwidth}
\begin{minipage}[b]{10cm}
\includegraphics[width=10cm]{images/BIG_editorAuthz002V5.PNG}
\tiny \emph{Note: package names had been partially blanked out for double-blind review.}
\vspace*{-2mm}
\captionof{figure}{A metamorphic relation for the Bypass Authorization Schema vulnerability.}
\label{fig:mrExample}
\end{minipage}
\hspace{5mm}
\begin{minipage}[b]{7cm}
\input{tables/grammar.tex}
\end{minipage}
\end{minipage}
\end{figure*}

==> tables/grammar.tex <==

\scriptsize

\begin{tabular}{|@{\hspace{0.1cm}}p{0.2cm} | @{\hspace{0.05cm}}p{6.5cm} |}
\LLRESET
\LL &\textbf{grammar} lang.SMRL \textbf{with} org.eclipse.xtext.xbase.Xbase\\
\LL &\textbf{import} "http://www.eclipse.org/xtext/xbase/Xbase" \textbf{as} xbase
\vspace{1mm}\\ 
\LL &SMRL:\\
\LL &\hspace{2mm}    importSection=XImportSection?\manuallabel{fig:grammar:importSec}{\LINE}\\
\LL &\hspace{2mm}    elements+=AbstractElement*;\\
\LL &AbstractElement:\\
\LL &\hspace{2mm}    PackageDeclaration $|$ MR;
\vspace{1mm}\\
\LL & PackageDeclaration:\manuallabel{fig:grammar:package}{\LINE}\\
\LL &\hspace{2mm}    `package` name=QualifiedName '\{' \\
\LL &\hspace{8mm}        elements+=AbstractElement*\\
\LL &\hspace{2mm}    '\}';
\vspace{1mm}\\ 
\LL &MR:\\
\LL &\hspace{2mm}    `MR` name=ValidID '\{'\manuallabel{fig:grammar:MRstart}{\LINE}\\
\LL &\hspace{8mm}        operations+=Operation\\
\LL &\hspace{2mm}    '\}';
\vspace{1mm}\\
\LL &Operation:\\
\LL &\hspace{2mm}   body=XBlockExpression;\manuallabel{fig:grammar:XEXPR}{\LINE}\\
\end{tabular}
\captionof{figure}{The \SMRL grammar.}
\label{tab:grammar}


==> tables/tableResults.tex <==





\begin{table}[tb]
\scriptsize
\caption{Summary of RQ2 results grouped by data collection method.}
\begin{tabular}{|@{\hspace{0.1cm}}p{1.6cm} | @{\hspace{0.05cm}}p{1.5cm} |  @{\hspace{0.05cm}}p{11mm} | @{\hspace{0.05cm}}p{8mm}    |  @{\hspace{0.05cm}}p{11mm} | @{\hspace{0.05cm}}p{8mm} |  }
\hline
\multirow{3}{*}{\textbf{Case study}}&\multirow{3}{*}{\textbf{Vulnerabilities}}&\multicolumn{4}{c|}{\textbf{Data collection method}}\\
&&\multicolumn{2}{c}{\textbf{Crawljax}}&\multicolumn{2}{c|}{\textbf{Crawljax \& Manual}}\\
&&\textbf{Precision}&\textbf{Recall}&\textbf{Precision}&\textbf{Recall}\\
\hline
\IWS	& 5& 1.0 & 0.80 & 1.0 & 1.0\\
\hline
Jenkins 2.121.1	& \JVulnUsed \cite{JV1,JV2,JV3,JV4,JV5,JV6,JV8,JV9}& 1.0 & 0.50 &   1.0 & 0.75  \\
\hline
\textbf{Overall} & 13 & 1.0 & 0.70 &   1.0 & 0.85  \\
\hline
\end{tabular}
\label{table:resultsRQ2}
\end{table}%






==> tables/tableVulnerabilityDetails.tex <==
\begin{table}[tb]
\scriptsize
\caption{Discovered vulnerabilities grouped by OWASP ID.}
\begin{tabular}{|p{2cm} | p{6mm} | p{18mm} | p{17mm} | }
\hline
\textbf{Vulnerability}&\multicolumn{3}{c|}{\textbf{\# Vulnerabilities Discovered}} \\
&\textbf{IWS}& \textbf{Jenkins 2.121.1} & \textbf{Jenkins 2.120} \\
\hline

OTG-AUTHN-001 &\TENT{1} &  \TENT{-} & \TENT{-} \\
OTG-AUTHN-003 &\TENT{-} &  \TENT{1} & \TENT{-} \\
OTG-AUTHN-004 &\TENT{1} &  \TENT{-} & \TENT{-} \\

OTG-AUTHZ-001&\TENT{1} &  \TENT{3} & \TENT{1} \\
OTG-AUTHZ-002 &\TENT{1} &  \TENT{4} & \TENT{1} \\

OTG-AUTHZ-004&\TENT{1} &  \TENT{-} & \TENT{-} \\
OTG-SESS-003 &\TENT{-} &  \TENT{1} & \TENT{-} \\

\hline
\end{tabular}
\\
\begin{minipage}{8.3cm}
\footnotesize{\textbf{Note}: a dash (-) indicates that the vulnerability does not affect the system.}
\end{minipage}
\label{table:resultsRQ2vulns}
\end{table}%





